Global-Local Self-Distillation for Visual Representation Learning

The downstream accuracy of self-supervised methods is tightly linked to the proxy task solved during training and the quality of the gradients extracted from it. Richer and more meaningful gradients updates are key to allow self-supervised methods to learn better and in a more efficient manner. In a typical self-distillation framework, the representation of two augmented images are enforced to be coherent at the global level. Nonetheless, incorporating local cues in the proxy task can be beneficial and improve the model accuracy on downstream tasks. This leads to a dual objective in which, on the one hand, coherence between global-representations is enforced and on the other, coherence between local-representations is enforced. Unfortunately, an exact correspondence mapping between two sets of local-representations does not exist making the task of matching local-representations from one augmentation to another non-trivial. We propose to leverage the spatial information in the input images to obtain geometric matchings and compare this geometric approach against previous methods based on similarity matchings. Our study shows that not only 1) geometric matchings perform better than similarity based matchings in low-data regimes but also 2) that similarity based matchings are highly hurtful in low-data regimes compared to the vanilla baseline without local self-distillation. The code is available at https://github.com/tileb1/global-local-self-distillation.

==> fig/first_fig.tex <==
\begin{figure*}[t!]
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{fig/cvpr.drawio.png}

   \caption{\textbf{Example of our inverse distance-based weighted local-representation matching between 2 augmentations of an input image.} Each location on a coarse grained grid (corresponding to the area of an output token) on the right image is linked to the best matching location on the left image based on the distance between the center of the locations. The size of the matching line corresponds to the weighting which is computed relatively to all others matching distances. The smaller the matching distance is in the input image, the higher the weighting is. Colors are used only to better differentiate different matchings.}
   \label{fig:first_fig}
\end{figure*}



==> fig/global-local_loss.tex <==
% \begin{figure}[h]
%   \centering
%   %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=\linewidth]{fig/eccv.drawio.pdf}

%   \caption{\textbf{Visual illustration of global-local objective framework with a loss for each component.} The global loss maximizes the similarity of both global-representations while the local losses maximize the similarity between pairs of local-representations.}
%   \label{fig:global-local_loss}
% \end{figure}

==> fig/scale_temp_ablation.tex <==
\begin{figure}[t]
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{fig/scale_temp_ablation_hingeFalse.pdf}

   \caption{\textbf{Ablation of the scale temperature hyperparameter $\tau_s$ (trained using point \ref{weighting_d} and \ref{scale_discrepancies} from \cref{sec:weighted-local-representation-loss}).} All methods are trained for 100 epochs with the same 100k image split of ImageNet \cite{imagenet} and evaluated on the original validation set.}
   \label{fig:scale_temp_ablation}
\end{figure}

==> sections/limitations.tex <==
\section{Limitations}
\label{sec:limitations}
Given the much higher performance in low-data regimes, one could assume that the convergence over EsViT would be faster when trained on the full dataset. Interestingly, it is not the case and the convergence speeds are very similar as can be seen from the convergence plot in the appendix.
Secondly, due to limited compute resources, we were not able to train for 300 epochs, or on other datasets. 
% \input{fig/epochs}

==> tab/comparison_of_methods.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c}
\hline
\textbf{Method} & \textbf{Backbone} & $\mathbf{\mathcal{L}_G}$   & $\mathbf{\mathcal{L}_L}$    & \textbf{Matching type} & \textbf{Data-augmentations} \\
\hline
BYOL \cite{byol}  & ResNet   & MSE           &       \xmark        &     \xmark                & base                  \\
DINO  \cite{dino} & ViT      & XENT &          \xmark     &  \xmark                   & base + multi-crop     \\
EsViT \cite{esvit} & Swin     & XENT & XENT & similarity          & base + multi-crop     \\
SPADE (ours) & Swin     & XENT & XENT & weighted distance   & base + multi-crop    
\end{tabular}
}
\caption{\textbf{Rough comparison of methods based on several components.} $\mathcal{L}_G$ and $\mathcal{L}_L$ refer respectively to the global- and local-representation loss. XENT and MSE refer respectively to cross entropy and mean squared error. The matching type column refers to the matching in the local-representation loss.}
\label{tab:rough_comparison}
\end{table}

==> tab/table_compute_similarity.tex <==
% \begin{table}[t]
% \centering
% \caption{\textbf{Comparison of similarity matchings of local-representations $\dense_k$ for all subsets of training data.} }

% % \resizebox{0.85\columnwidth}{!}{%
% % \begin{tabular}{l|c|c}
% % \hline
% % \textbf{Method} & \textbf{Accuracy} & \textbf{Error} \\
% % \hline
% % Random init \& no training  & 0.346    & 70.71 \\
% % EsViT  & 0.920    & 4.084 \\

% % SPADE & 0.921    & 3.921 \\
% % % SPADE ($\tau_d=0.1$)  & 0.923    & 3.795 \\
% % % test & \multicolumn{2}{c}{test}



% % \end{tabular}
% % }

% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|c|cccccc}
% \hline
% \textbf{Method} & \textbf{Metric}     & \textbf{1\%}   & \textbf{2\%}   & \textbf{5\%}   & \textbf{10\%}  & \textbf{20\%}  & \textbf{100\%}\\
% \hline
% \texttt{Vanilla}  & Accuracy [\%] & 59.5 & 71.4 & 86.0 & 91.4 & 86.3 & 85.4 \\
% \texttt{Similarity}  & Accuracy [\%] & 3.40 & 20.0 & 52.5 & 88.7 & 92.3 & 89.5 \\
% \texttt{Geometric}  & Accuracy [\%] & 69.3 & 79.6 & 89.2 & 91.3 & 93.1 & 89.8 \\
% \hline
% \texttt{Vanilla}  & Error  [pixel]  & 36.90 & 23.90 & 10.06 & 5.426 & 9.55 & 11.25 \\
% \texttt{Similarity}  & Error  [pixel]  & 112.5 & 79.00 & 37.92 & 6.855 & 4.184 & 7.744 \\
% \texttt{Geometric}  & Error  [pixel]  & 26.38 & 16.24 & 7.313 & 5.179 & 3.724 & 7.054
% \end{tabular}
% % }
% \label{tab:compute_similarity}
% \end{table}



% Total accuracy: 0.9214923977851868, Total error: 3.921531915664673 (29)
% Total accuracy: 0.9205277562141418, Total error: 4.0849456787109375
%Total accuracy: 0.34698477387428284, Total error: 70.71449279785156


% \resizebox{0.75\columnwidth}{!}{%
% \begin{tabular}{l|c|c}
% \hline
% \textbf{Method} & \textbf{Accuracy} & \textbf{Error} \\
% \hline
% Random init \& no training  & 0.346    & 70.71 \\
% EsViT  & 0.920    & 4.084 \\

% SPADE ($\tau_d=0.1$ and using hinge)  & 0.921    & 3.921 \\
% SPADE ($\tau_d=0.1$)  & 0.923    & 3.795 \\
% % test & \multicolumn{2}{c}{test}



% \end{tabular}
% }
